Revisiting Human Information Foraging: Adaptations for LLM-based Chatbots

Information Foraging Theory's (IFT) framing of human information seeking choices as decision-theoretic cost-value judgments has successfully explained how people seek information among linked patches of information (e.g., linked webpages). However, the theory has to be adopted and validated in non-patchy LLM-based chatbot environments, before its postulates can be reliably applied to the design of such chat-based information seeking environments. This paper is a thought experiment that applies the IFT cost-value proposition to LLM-based chatbots and presents a set of preliminary hypotheses to guide future theory-building efforts for how people seek information in such environments.

==> sections/gaps.tex <==
\section{Perception and mastery: components missing in IFT}
\label{sec:gap}

IFT is mostly concerned with finding or using the information found. However, it ignores the learning/development behavior of the worker. In classical IFT, the performance of a user in foraging was tied to their mastery in the field and their skills in effective evaluation and synthesis of different isolated information sources. The effortful foraging process could encourage the user to   

\textbf{Mastery}: Mastery refers to a high level of expertise or skill in a particular field. It is characterized by deep understanding, proficiency, and the ability to apply knowledge and techniques effectively. Achieving mastery often requires extensive practice, study, and experience, as well as a commitment to continuous learning and improvement.

